Fast and Complete: Enabling Complete Neural Network Verification with Rapid and Massively Parallel Incomplete Verifiers

Formal verification of neural networks (NNs) is a challenging and important problem. Existing efficient complete solvers typically require the branch-and-bound (BaB) process, which splits the problem domain into sub-domains and solves each sub-domain using faster but weaker incomplete verifiers, such as Linear Programming (LP) on linearly relaxed sub-domains. In this paper, we propose to use the backward mode linear relaxation based perturbation analysis (LiRPA) to replace LP during the BaB process, which can be efficiently implemented on the typical machine learning accelerators such as GPUs and TPUs. However, unlike LP, LiRPA when applied naively can produce much weaker bounds and even cannot check certain conflicts of sub-domains during splitting, making the entire procedure incomplete after BaB. To address these challenges, we apply a fast gradient based bound tightening procedure combined with batch splits and the design of minimal usage of LP bound procedure, enabling us to effectively use LiRPA on the accelerator hardware for the challenging complete NN verification problem and significantly outperform LP-based approaches. On a single GPU, we demonstrate an order of magnitude speedup compared to existing LP-based approaches.

==> notation_table.tex <==
\begin{table}[]
    \centering
    \caption{Table of Notations\textcolor{red}{Huan: I think we can remove the table, it takes too much space, and many of them like $A, B, I, \gamma$ are not used anymore.}}
    \label{tab:notations}
    \begin{tabular}{p{1.5cm}|p{11cm}}
    \hline
         Symbol &  Meanings\\
         \hline
         $f(x)$ & Neural network function\\
         $l(x), u(x)$ & lower and upper bounds of function $f(x)$\\
         $W^i$ & Weight matrix of a linear transformation layer (convolutional/fully-connected)\\
        %  \textcolor{Lin_color}{fully-connected})\\
         $z^i$ & Pre-activation output of layer $i$\\
         $h(\cdot)$ &Non-linear activation function\\
         $x^i$ & Layer $i + 1$'s input, $x^i = h(z^i)$ %where $h(\cdot)$ is a non-linear activation function 
         \\
        %  $x^0$ & Input of the neural network\\
        %  $x^o$ & Output of the neural network\\
         $\gamma_l$, $\gamma_u$ & Lower and upper bounds of an arbitrary variable $\gamma$\\
         $A^i_l, A^i_u$ & Linear coefficients of $x^i$ in the linear lower and upper bounds of $y$\\
         $B^i_l, B^i_u$ & Bias terms of the linear lower and upper bounds between layer $i$ inputs $x^i$ and output $y$\\
         $I_+^i, I_-^i, I^i$ & Set of active, dead and uncertain ReLU neurons between layer $i$ and layer $i + 1$, respectively\\
         $\gC, \gC_i$ & Bounded input domain and $i$th split sub-domain\\
        %  & \LX{about should be "$\{I_+^i, I_-^i, I^i\}$"? two $I_+^i$ used above}\\
    \hline
    \end{tabular}
\end{table}
\vspace{-1em}

